On the (Parameterized) Complexity of Almost Stable Marriage

In the Stable Marriage problem. when the preference lists are complete, all agents of the smaller side can be matched. However, this need not be true when preference lists are incomplete. In most real-life situations, where agents participate in the matching market voluntarily and submit their preferences, it is natural to assume that each agent wants to be matched to someone in his/her preference list as opposed to being unmatched. In light of the Rural Hospital Theorem, we have to relax the "no blocking pair" condition for stable matchings in order to match more agents. In this paper, we study the question of matching more agents with fewest possible blocking edges. In particular, we find a matching whose size exceeds that of stable matching in the graph by at least t and has at most k blocking edges. We study this question in the realm of parameterized complexity with respect to several natural parameters, k,t,d, where d is the maximum length of a preference list. Unfortunately, the problem remains intractable even for the combined parameter k+t+d. Thus, we extend our study to the local search variant of this problem, in which we search for a matching that not only fulfills each of the above conditions but is "closest", in terms of its symmetric difference to the given stable matching, and obtain an FPT algorithm.

==> w-hardness.tex <==
% !TEX root = NASM-main.tex


\section{Construction Used in Theorem~\ref{thm:smd w-hard}}
%Proof of Theorem~\ref{thm:smd w-hard}}
%\paragraph{Theorem~\ref{thm:smd w-hard}.}
%{\it \ams is \WOH with respect to $k+q+t$.}
%\end{theo}
In this section we give a construction of  polynomial-time reduction from \mcqsmall.
 %similar to the one in Theorem~\ref{thm:asm}. 
The detailed description of the construction of an instance of \ams is as follows. 

 {\bf Construction.} Given an instance $(G,(V_1,\cdots,V_k))$ of \mcqsmall, we construct an instance $(G',\pref,\mu,k',q,t)$ of \ams as follows.  
 %Figure \ref{fig:hardness} describes the construction of $G'$. 
\begin{sloppypar}
\begin{itemize}[noitemsep]
\item For each $i \in [k]$ and for each vertex $v\in V_i$, we add a path on four vertices namely, $(v^i_1,v^i_2,v^i_3,v^i_4)$ in $G'$. %Let $u\in V_i$ and $v\in V_j$, where $\{i,j\}\subseteq [k]$, and $i<j$. 
\item For each edge $e \in E(G)$ with endpoints $u \in V_i$ and $v \in V_j$ %(since $V_i$ and $V_j$ are independent sets)
 where $i<j$, we add vertices $e_1^{ij}$ and $e_2^{ij}$ to $V(G')$, and an edge $e_1^{ij}e_2^{ij}$ to $E(G')$.  %Now, f
\item For each $i\in[k]$, we add two vertices $p_1^i, p_2^i$, and for each $\{i,j\} \subseteq [k]$ where $i<j$,  we add two vertices $q_1^{ij}, q_2^{ij}$ to $V(G')$. 
\item %We %also add 
For each $i\in[k]$ and for each vertex $u \in V_i$, we add two edges $u^i_1p_1^i$ and $u^i_4p_2^i$ to $E(G')$. %let $Z_1^i=\{u^i_1p_1^i,u^i_4p_2^i\colon u\in V_i\}$.
 For each $\{i,j\} \subseteq [k]$ and for each edge $e \in E(G)$ with endpoints $u \in V_i$ and $v \in V_j$ where $i<j$, we add four edges $q_1^{ij}e_1^{ij}, q_2^{ij}e_2^{ij}, e_1^{ij}u_3^{i}$, and $ e_1^{ij}v_3^{j}$ to $E(G')$.  
 \end{itemize}
\end{sloppypar}
Note that $V(G')=4\lvert V(G)\rvert+2\lvert E(G)\rvert+2k+k(k-1)$. 
%Recall that in earlier reduction, for each vertex in $V(G)$, we added a path of length $2r+2$, while here we add a path of length $4$. Moreover, instead of adding $n$ vertices $p_{\ell}^i$ and $\tilde{p}_\ell^i$, for each $i\in [k]$, we only add two vertices $p_1^i$ and $p_2^i$. Similarly, we added only two vertices $q_1^{ij}$ and $q_2^{ij}$ instead of adding $m$ such vertices. Furthermore, we did not add many vertices which we added in previous reduction. This is how we decrease the length of augmenting paths. But, note that degree of vertices $u_3^i$, where $u\in V_i$, $p_1^i, p_2^i,q_1^{ij},q_2^{ij}$, where $\{i,j\}\subseteq [k]$, is large.
 
 %let $Z_2^{ij}=\{q_1^{ij}e_1^{ij}, q_2^{ij}e_2^{ij}, e_1^{ij}u_3^{i}, e_1^{ij}v_3^{j}\colon e(=uv)\in E(G),u\in V_i, v\in V_j, \text{ and } i<j\}$. We add $Z_1^i$ and $Z_2^{ij}$ to $E(G')$, for all $i\in[k]$ and $\{i,j\} \subseteq [k]$, where $i<j$. 
 %Then, $E(G')=Z_1\cup Z_2$. %If $u\in V_i$, then add edges $u^i_1p_1^i$ and $u^i_4p_2^i$ to $E(G')$. For each $\{i,j\} \subseteq [k]$, we add two vertices $q_1^{ij}$ and $q_2^{ij}$ to $V(G')$. Let $u\in V_i$ and $v\in V_j$, where $\{i,j\}\subseteq [k]$. If $e=uv\in E(G)$, then add edges $q_1^{ij}e_1^{ij}$, $q_2^{ij}e_2{ij}$, $e_1^{ij},u_3^{i}$, and $e_2^{ij},v_3^{i}$ to $E(G')$.  

For each $i \in [k]$ and each vertex $u\in V_i$, we define $S_u=\{e_1^{ij}\colon e(=uv)\in E(G) \text{ for some } v\in V_j, j \in [k] \setminus \{i\}\}$.   The preference list of each vertex in $G'$ is presented in Table \ref{pref_list}.

%\begin{figure*}
%    \centering
%%\includegraphics[width=15cm,height=105cm,keepaspectratio]{fig_hardness.pdf}
%\includegraphics[width=15cm,height=3cm]{fig_hardness.pdf}
%\caption{An illustration of construction of graph $G'$ in \W[1]-hardness of \ams. Here, {\color{blue} blue} colored edges belongs to the stable matching $\mu$. Note that $u,v,w,x,y,z,r,s,$ and $t$ are vertices of $G$ and $e$ and $\hat{e}$ are edges of $G$.
%}\label{fig:hardness}
%\end{figure*}



 %V(G) \text{ and } \{u,v\}\subseteq V_i\cup V_j, \{i,j\}\subseteq [k]\}$. Now, we assign preference list to each vertex in $G'$ as shown in Table \ref{pref_list}. %In the preference list (Table \ref{pref_list}), the symbol $[S]$ denotes that the vertices in the set $S$ are listed in some arbitrarily strict order. 
% For each $u\in V(G)$, let $S_u=\{e_1^{ij}\colon e(=uv)\in E(G) \text{ for some } v\in V(G) \text{ and } \{u,v\}\subseteq V_i\cup V_j, \{i,j\}\subseteq [k]\}$.
% For each $u\in V_i$, $i\in[k]$, let $S_u=\{e_1^{ij}\colon e(=uv)\in E(G) \text{ for some } v\in V_j, j\in[k]\}\cup \{e_1^{ji}\colon e(=uv)\in E(G) \text{ for some } v\in V_j, j\in[k]\}$. %Let $S_{p_1^i}=\{u_1^i\colon u\in V_i\}$ and $S_{p_2^i}=\{u_4^i\colon u\in V_i\}$, where $i\in [k]$. %Let $u\in V_i$ and $v\in V_j$. For an edge $e=(uv)$, $S[e]=\{u_3^i,v_3^i\}$
%For each $\{i,j\}\subseteq [k]$, where $i<j$, $S_{q_1^{ij}}=\{e_1^{ij}\colon e(=uv)\in E(G), u\in V_i, \text{ and } v\in V_j\}$ and  $S_{q_2^{ij}}=\{e_2^{ij}\colon e(=uv)\in E(G), u\in V_i, \text{ and } v\in V_j\}$.  
%Note that $G'$ is a bipartite graph as it does not contain any odd cycle.

 %Now, we will show that $G'$ is a bipartite graph.

%\noindent
{\bf $G'$ is bipartite:} A bipartition for $G'$ can be created by assigning $p_1^i$, $v^i_2$ and $v^i_4$ to one part and $p_2^i$, $v^i_1$ and $v^i_3$ to another part for each $i \in [k]$, and each $v \in V_i$. %, we add the vertices $v^i_1,v^i_2,v^i_3,v^i_4$ to partition two, one, two, one, respectively.
 For $\{i,j\} \subseteq [k]$, since $e_1^{ij}$ (corresponding to the edge $e=uv, u \in V_i, v \in V_j$) is connected to $u_3^i$ and $v_3^j$, we assign $e_1^{ij}$ and $q_2^{ij}$ to the  part containing $p_1^i$, and assign $e_2^{ij}$ and $q_1^{ij}$ to the part containing $p_2^i$. Observe that each part is an independent set. Hence $G'$ is a bipartite graph. 
 %Next, we construct a stable matching $\mu$. 
%\noindent

{\bf Stable matching $\mu$:} Let $\mu=\{u_1^iu_2^i, u_3^iu_4^i, e_1^{ij}e_2^{ij}\colon \{i,j\}\subseteq [k]\}$. Note that $\lvert \mu\rvert = 2\lvert V(G)\rvert +\lvert E(G)\rvert$. We will show that $\mu$ is a stable matching.  Note that $u_1^i$ and $u_2^i$ prefer each other over any other vertex in $G'$. Therefore, $u_1^iu_2^i$ belongs to every stable matching of $G'$. Similarly, since $e_1^{ij}$ and $e_2^{ij}$ prefer each other over any other vertex, $e_1^{ij}e_2^{ij}$ belongs to every stable matching of $G'$. %Let $\mu=\{u_1^iu_2^i, u_3^iu_4^i, e_1^{ij}e_2^{ij}\colon \{i,j\}\subseteq [k]\}$. 
 Since $u_3^i$ is the first preference of $u_4^i$, and the vertices which  $u_3^i$ prefers over $u_4^i$ ( i.e., $u_2^i$ and vertices in $S_u$) are matched to their first preferred vertices, it follows that $\mu$ is a stable matching in $G'$.
 
 %{\color{red} Observe that  $u_1^iu_2^i$ and $ e_1^{ij}e_2^{ij}$ are must be in every stable matching of $G'$, since $u_1^i$ ( or $e_1^{ij}$) and $u_2^i$ (or $e_2^{ij}$) prefer each other over every other vertex. Hence,  $\mu$ is the unique stable matching in $G'$.} 
 %Since for each $u\in V(G)$, $\{u_1^iu_2^i, u_3^iu_4^i\}\subseteq \mu$ and for each $e\in E(G)$, $e_1^{ij}e_2^{ij}\in \mu$, the size of $\mu$ is $2n+m$. 


{\bf Parameter:} We set $k'=k+\nicefrac{k(k-1)}{2}$, $q=5k+\nicefrac{3k(k-1)}{2}$, and $t=k'$.  
Clearly, this construction can be carried out in polynomial time. %Due to paucity of space the proof of correctness is deferred to Appendix~\ref{sec:wh_proof}. %due to paucity of space.
% Requires the booktabs if the memoir class is not being used
%\begin{table}[htbp]
\begin{table}[t]
   \centering
 % \begin{tabularx}{\textwidth}{@{} lcl @{} lcl @{}} 
	\begin{tabularx}{\textwidth}{ C{0.1cm}  C{3.2cm}  C{4cm}} 
    $u_1^i \colon$ & $u_2^i,p_1^i$ & $i\in[k]$\\
    $u_2^i \colon$ & $u_1^i,u_3^i$ & $i\in[k]$\\
    $u_3^i \colon$ & $u_2^i,\langle S_u \rangle,u_4^i$ & $i\in [k]$\\
    $u_4^i \colon$ & $u_3^i,p_2^i$ & $i\in[k]$ \\
    $p_1^i \colon$ & $\langle N(p_1^i) \rangle$%[S_{p_1^i}]$ 
    & $i\in [k]$ \\
    $p_2^i \colon$ & $\langle N(p_2^i) \rangle$ & $i\in [k]$ \\ 
    $e_1^{ij}\colon$ & $e_2^{ij},u_3^i,v_3^j, q_1^{ij}$ & $ e=uv, 
    u\in V_i, v\in V_j, \{i,j\}\subseteq [k], \text{ and } i<j$\\
    $e_2^{ij}\colon$ & $e_1^{ij}, q_2^{ij}$ & $\{i,j\}\subseteq [k], i<j$\\
    $q_1^{ij}\colon$ & $\langle N(q_1^{ij}) \rangle$ & $\{i,j\}\subseteq [k], i<j$\\
    $q_2^{ij}\colon$ & $\langle N(q_2^{ij}) \rangle$ & $\{i,j\}\subseteq [k], i<j$\\
    \end{tabularx}
   \caption{Preference lists in the constructed instance of \textsf{\textup{W[1]-hardness}} of \ams when parameterized by $k+q+t$. Here, the symbol $\langle S \rangle$ denotes that the vertices in the set $S$ are listed in some arbitrarily strict order. }
   \label{pref_list}
\end{table}

%We show the equivalence between the instance $(G,k)$ of \mcqsmall and $(G',\pref,\mu,k',q,t)$ of \ams in the attached supplementary file. 

%\end{proof}
\input{w-hardness_proofnew}




 
 

